Fast Wavelet Decomposition of Linear Operators through Product-Convolution Expansions

Wavelet decompositions of integral operators have proven their efficiency in reducing computing times for many problems, ranging from the simulation of waves or fluids to the resolution of inverse problems in imaging. Unfortunately, computing the decomposition is itself a hard problem which is oftentimes out of reach for large scale problems. The objective of this work is to design fast decomposition algorithms based on another representation called product-convolution expansion. This decomposition can be evaluated efficiently assuming that a few impulse responses of the operator are available, but it is usually less efficient than the wavelet decomposition when incorporated in iterative methods. The proposed decomposition algorithms, run in quasi-linear time and we provide some numerical experiments to assess its performance for an imaging problem involving space varying blurs.

==> images/timings_fKernel_6_error.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.856\textwidth,
height=0.9\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmode=log,
xmin=1e-12,
xmax=100,
xminorticks=true,
ymode=log,
ymin=7.273938,
ymax=10000,
yminorticks=true,
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid]
  table[row sep=crcr]{%
1.67501726218833e-11	2744.650428\\
1.67364628533338e-11	2801.430133\\
1.67527812506847e-11	2607.87298\\
1.67762119939259e-11	2543.006774\\
1.67456386191878e-11	2482.692712\\
1.67714968510424e-11	2425.723949\\
1.67844326561904e-11	2361.225302\\
1.67375293035589e-11	2299.003097\\
1.68909903039785e-11	2231.252402\\
1.80784221382015e-11	2162.941625\\
2.24120703660194e-11	2201.88666\\
3.70055216859638e-11	2010.644929\\
7.36275248607216e-11	1927.169559\\
1.5445904319607e-10	1840.186374\\
3.22143260858928e-10	1748.75678\\
6.96059473236566e-10	1651.711343\\
1.45499484995441e-09	1547.723732\\
3.05141215816243e-09	1443.06721\\
6.35300771649496e-09	1327.119255\\
1.34362259091326e-08	1213.192979\\
2.82732088994837e-08	1098.710265\\
5.89040027061174e-08	982.721583\\
1.23992415430655e-07	871.699326\\
2.52252663043278e-07	761.528742\\
5.1168061939953e-07	654.597466\\
1.01015836286354e-06	646.319091\\
2.09074516630877e-06	479.446291\\
4.24367780382086e-06	382.470091\\
8.41055525408891e-06	310.600171\\
1.73531098477289e-05	248.834622\\
3.55930216754963e-05	200.487555\\
7.32998068300962e-05	155.392744\\
0.00015080789129171	121.5648\\
0.000299616042322034	95.227028\\
0.000597828534686361	75.330738\\
0.00112655466092415	58.862097\\
0.00214649449839959	47.946383\\
0.00398225677917674	38.736334\\
0.00719012773593595	32.272336\\
0.0127089325717889	26.691588\\
0.0221156832147235	22.729819\\
0.0367742714766127	19.641446\\
0.0590945642506985	16.90793\\
0.0959386808917537	15.685182\\
0.143390801836229	13.767977\\
0.227421695294071	13.262766\\
0.400282193225295	11.018766\\
0.608285049166736	9.66555\\
1.00833533644395	8.716306\\
1.01648109450941	7.273938\\
};
\addlegendentry{Decomposition time};

\addplot [color=mycolor2,solid]
  table[row sep=crcr]{%
1.67501726218833e-11	3525.26715682524\\
1.67364628533338e-11	3525.92289174699\\
1.67527812506847e-11	3525.14246132057\\
1.67762119939259e-11	3524.02351148659\\
1.67456386191878e-11	3525.48394416756\\
1.67714968510424e-11	3524.24853189824\\
1.67844326561904e-11	3523.631382984\\
1.67375293035589e-11	3525.87186005064\\
1.68909903039785e-11	3518.56977358102\\
1.80784221382015e-11	3464.68773066058\\
2.24120703660194e-11	3299.63876578451\\
3.70055216859638e-11	2944.40305780974\\
7.36275248607216e-11	2518.44039838475\\
1.5445904319607e-10	2128.34403666119\\
3.22143260858928e-10	1801.06071867102\\
6.96059473236566e-10	1511.90859886709\\
1.45499484995441e-09	1278.76162001128\\
3.05141215816243e-09	1080.76213756092\\
6.35300771649496e-09	914.931627747512\\
1.34362259091326e-08	771.788231163429\\
2.82732088994837e-08	651.789577397427\\
5.89040027061174e-08	551.695938218717\\
1.23992415430655e-07	465.880362185568\\
2.52252663043278e-07	396.472434178698\\
5.1168061939953e-07	337.63056449593\\
1.01015836286354e-06	289.297479823384\\
2.09074516630877e-06	245.237131313615\\
4.24367780382086e-06	208.810251633827\\
8.41055525408891e-06	178.760035274047\\
1.73531098477289e-05	151.642417478957\\
3.55930216754963e-05	128.811199100618\\
7.32998068300962e-05	109.317311463933\\
0.00015080789129171	92.7937917223344\\
0.000299616042322034	79.3957121415222\\
0.000597828534686361	67.8656914976971\\
0.00112655466092415	58.7685429342884\\
0.00214649449839959	50.7631816298403\\
0.00398225677917674	44.1146320614301\\
0.00719012773593595	38.5740321615692\\
0.0127089325717889	33.8926159713719\\
0.0221156832147235	29.8851520613397\\
0.0367742714766127	26.6251125629072\\
0.0590945642506985	23.9055289554873\\
0.0959386808917537	21.413916490723\\
0.143390801836229	19.5457649507645\\
0.227421695294071	17.6016221275277\\
0.400282193225295	15.4803317317277\\
0.608285049166736	14.076618639743\\
1.00833533644395	12.5498934501786\\
1.01648109450941	12.5269779844864\\
};
\addlegendentry{data1};

\end{axis}
\end{tikzpicture}%
